BEHRT: Transformer for Electronic Health Records

Today, despite decades of developments in medicine and the growing interest in precision healthcare, vast majority of diagnoses happen once patients begin to show noticeable signs of illness. Early indication and detection of diseases, however, can provide patients and carers with the chance of early intervention, better disease management, and efficient allocation of healthcare resources. The latest developments in machine learning (more specifically, deep learning) provides a great opportunity to address this unmet need. In this study, we introduce BEHRT: A deep neural sequence transduction model for EHR (electronic health records), capable of multitask prediction and disease trajectory mapping. When trained and evaluated on the data from nearly 1.6 million individuals, BEHRT shows a striking absolute improvement of 8.0-10.8%, in terms of Average Precision Score, compared to the existing state-of-the-art deep EHR models (in terms of average precision, when predicting for the onset of 301 conditions). In addition to its superior prediction power, BEHRT provides a personalised view of disease trajectories through its attention mechanism; its flexible architecture enables it to incorporate multiple heterogeneous concepts (e.g., diagnosis, medication, measurements, and more) to improve the accuracy of its predictions; and its (pre-)training results in disease and patient representations that can help us get a step closer to interpretable predictions.

==> prec_table.tex <==
\begin{longtable}[h]{|p{1cm}|p{1.2cm}|p{1.2cm}|p{4.5cm}|p{1.5cm}|p{4.5cm}|}
\caption{Diseases Prediction Performance }\\
 \hline
Caliber &  APS &  AUROC & Description & Ratio & Caliber Chapter \\
 \hline
 \endhead
  92 &  0.066765 &  0.723828 &  Gastritis and duodenitis &  0.011198 &  Diseases of the digestive system \\
  66 &  0.108185 &  0.797633 &  Diaphragmatic hernia &  0.011490 &  Diseases of the digestive system \\
  100 &  0.118093 &  0.742646 &  Hearing loss &  0.021964 &  Diseases of the ear and mastoid process \\
  273 &  0.132567 &  0.773249 &  Spondylosis &  0.013459 &  Diseases of the musculoskeletal system and connective tissue \\
  189 &  0.142594 &  0.844596 &  Pleural effusion &  0.010229 &  Diseases of the respiratory system \\
  172 &  0.162186 &  0.798654 &  Other anaemias &  0.023303 &  Diseases of the blood and blood-forming organs and certain disorders involving the immune mechanism \\
  29 &  0.163355 &  0.822707 &  Bacterial Diseases (excl TB) &  0.023979 &  Certain infectious and parasitic diseases   \\
  130 &  0.167457 &  0.804545 &  Iron deficiency anaemia &  0.020780 &  Diseases of the blood and blood-forming organs and certain disorders involving the immune mechanism \\
  295 &  0.169674 &  0.836610 &  Urinary Tract Infections &  0.022534 &  Diseases of the genitourinary system \\
  69 &  0.170852 &  0.811759 &  Diverticular disease of intestine (acute and chronic) &  0.015966 &  Diseases of the digestive system \\
  8 &  0.177170 &  0.810068 &  Allergic and chronic rhinitis &  0.023241 &  Diseases of the respiratory system \\
  170 &  0.181182 &  0.847938 &  Osteoporosis &  0.013982 &  Diseases of the musculoskeletal system and connective tissue \\
  71 &  0.184000 &  0.790655 &  Dyslipidaemia &  0.026010 &  Endocrine, nutritional and metabolic diseases \\
  168 &  0.184629 &  0.799592 &  Oesophagitis and oesophageal ulcer &  0.022426 &  Diseases of the digestive system \\
  217 &  0.203218 &  0.855593 &  Primary Malignancy Other Skin and subcutaneous tissue &  0.012013 &  Neoplasms \\
  93 &  0.206455 &  0.776367 &  Gastro-oesophageal reflux disease &  0.026271 &  Diseases of the digestive system \\
  290 &  0.208524 &  0.814481 &  Type 1 Diabetes Mellitus, Type 2 Diabetes Mellitus, and Diabetes Mellitus – other or not specified &  0.021226 &  Endocrine, nutritional and metabolic diseases \\
  3 &  0.219637 &  0.869366 &  Actinic keratosis &  0.012490 &  Diseases of the skin and subcutaneous tissue \\
  131 &  0.220017 &  0.874319 &  Irritable bowel syndrome &  0.011182 &  Diseases of the digestive system \\
  294 &  0.223863 &  0.824114 &  Urinary Incontinence &  0.020057 &  Diseases of the genitourinary system \\
  169 &  0.234444 &  0.785766 &  Osteoarthritis (excl spine) &  0.043714 &  Diseases of the musculoskeletal system and connective tissue \\
  176 &  0.245906 &  0.834062 &  Other or unspecified infectious organisms &  0.030963 &  Diseases of the respiratory system \\
  95 &  0.249208 &  0.894444 &  Glaucoma &  0.011367 &  Diseases of the eye and adnexa \\
  109 &  0.250573 &  0.885547 &  Hyperplasia of prostate &  0.020842 &  Diseases of the genitourinary system \\
  184 &  0.264687 &  0.879325 &  Peripheral arterial disease &  0.010951 &  Diseases of the circulatory system \\
  79 &  0.265863 &  0.762939 &  Enthesopathies \& synovial disorders &  0.047036 &  Diseases of the musculoskeletal system and connective tissue \\
  81 &  0.267187 &  0.905812 &  Erectile dysfunction &  0.017873 &  Mental and behavioural disorders \\
  140 &  0.268504 &  0.867094 &  Lower Respiratory Tract Infections &  0.023518 &  Certain infectious and parasitic diseases   \\
  63 &  0.271027 &  0.753816 &  Dermatitis (atopc/contact/other/unspecified) &  0.049051 &  Diseases of the skin and subcutaneous tissue \\
  142 &  0.292598 &  0.893802 &  Macular degeneration &  0.010752 &  Diseases of the eye and adnexa \\
  274 &  0.296798 &  0.889236 &  Stable Angina &  0.032039 &  Diseases of the circulatory system \\
  57 &  0.301041 &  0.900088 &  Coronary heart disease not otherwise specified &  0.035177 &  Diseases of the circulatory system \\
  275 &  0.307238 &  0.911618 &  Stroke Not otherwise specified (NOS) &  0.023395 &  Diseases of the nervous system \\
  45 &  0.319433 &  0.863447 &  Cataract &  0.042099 &  Diseases of the eye and adnexa \\
  1 &  0.319972 &  0.845171 &  Abdominal Hernia &  0.019180 &  Diseases of the digestive system \\
  44 &  0.325143 &  0.843480 &  Carpal tunnel syndrome &  0.012013 &  Diseases of the nervous system \\
  101 &  0.334902 &  0.912117 &  Heart failure &  0.024918 &  Diseases of the circulatory system \\
  164 &  0.335131 &  0.879670 &  Obesity &  0.017442 &  Endocrine, nutritional and metabolic diseases \\
  22 &  0.348523 &  0.885055 &  Asthma &  0.026133 &  Diseases of the respiratory system \\
  97 &  0.349361 &  0.882694 &  Gout &  0.018058 &  Diseases of the musculoskeletal system and connective tissue \\
  65 &  0.350132 &  0.942604 &  Diabetic ophthalmic complications &  0.018919 &  Endocrine, nutritional and metabolic diseases \\
  147 &  0.368465 &  0.911541 &  Migraine &  0.012028 &  Diseases of the nervous system \\
  229 &  0.398842 &  0.904686 &  Psoriasis &  0.011751 &  Diseases of the musculoskeletal system and connective tissue \\
  17 &  0.410899 &  0.858498 &  Anxiety disorders &  0.041914 &  Mental and behavioural disorders \\
  146 &  0.433645 &  0.969406 &  Menorrhagia and polymenorrhoea &  0.015504 &  Diseases of the genitourinary system \\
  113 &  0.489456 &  0.905032 &  Hypo or hyperthyroidism &  0.047897 &  Endocrine, nutritional and metabolic diseases \\
  302 &  0.491672 &  0.855823 &  Vitamin B12 deficiency anaemia &  0.014489 &  Diseases of the blood and blood-forming organs and certain disorders involving the immune mechanism \\
  51 &  0.501496 &  0.923082 &  Chronic obstructive pulmonary disease (COPD) &  0.036869 &  Diseases of the respiratory system \\
  23 &  0.514881 &  0.901268 &  Atrial Fibrillation and flutter &  0.077629 &  Diseases of the circulatory system \\
  110 &  0.531597 &  0.819527 &  Hypertension &  0.200618 &  Diseases of the circulatory system \\
  61 &  0.542223 &  0.950442 &  Dementia &  0.024656 &  Mental and behavioural disorders \\
  62 &  0.553561 &  0.877904 &  Depression &  0.076876 &  Mental and behavioural disorders \\
  85 &  0.573880 &  0.934049 &  Female genital prolapse &  0.015781 &  Diseases of the genitourinary system \\
  220 &  0.575574 &  0.964776 &  Primary Malignancy Prostate &  0.011844 &  Neoplasms \\
  6 &  0.583305 &  0.952656 &  Alcohol Problems &  0.014535 &  Mental and behavioural disorders \\
  194 &  0.647243 &  0.955062 &  Polymyalgia Rheumatica &  0.013213 &  Diseases of the musculoskeletal system and connective tissue \\
  80 &  0.648763 &  0.977907 &  Epilepsy &  0.016104 &  Diseases of the nervous system \\
  \hline
\end{longtable} 
